Measurement of Gravitational Coupling between Millimeter-Sized Masses

We demonstrate gravitational coupling between two gold spheres of approximately 1mm radius and 90mg mass. By periodically modulating the source mass position at a frequency f=12.7mHz we generate a time-dependent gravitational acceleration at the location of the test mass, which is measured off resonance in a miniature torsional balance configuration. Over an integration time of 350 hours the test mass oscillator enables measurements with a systematic accuracy of 4E-11m/s^2 and a statistical precision of 4E-12m/s^2. This is sufficient to resolve the gravitational signal at a minimal surface distance of 400mum between the two masses. We observe both linear and quadratic coupling, consistent in signal strength with a time-varying 1/r gravitational potential. Contributions of non-gravitational forces could be kept to less than 10% of the observed signal. We expect further improvements to enable the isolation of gravity as a coupling force for objects well below the Planck mass. This opens the way for precision tests of gravity in a new regime of isolated microscopic source masses.

==> figures.tex <==
\begin{figure*}[htb]
\centering
\includegraphics[width=0.9\linewidth]{images/mt_sketch_paper1_l4c.png}
\caption[schematic]{(a) Schematic of the experiment. The torsion pendulum, which acts as transducer for gravitational acceleration, consists of two $r\approx1\,\mathrm{mm}$ gold spheres held at $40\,\mathrm{mm}$ center distance by a glass capillary. One mass serves as $m_t=90.7\,\mathrm{mg}$ test mass, the other $m_a=91.5\,\mathrm{mg}$ as counterbalance that provides vibrational noise common mode rejection. A $\varnothing4\,\mathrm{\upmu m}$ silica fiber provides a soft $f_0=3.6\,\mathrm{mHz}$ torsional resonance separated well from other degrees of freedom. The torsion angle is read out via an optical lever directed to a quadrant photodiode. Gravitational interaction is modulated by harmonically moving the $m_s=92.1\,\mathrm{mg}$ source mass (m\textsubscript{t}) at a frequency well above the torsion resonance ($f_{mod}=12.7\,\mathrm{mHz}$) by $ds\approx3\,\mathrm{mm}$ by means of a shear piezo. Direct electrostatic coupling is suppressed by discharging and a $150\,\mathrm{\upmu m}$ thick Faraday shield.
(b) Source mass on a 1 Euro Cent coin.
(c) Photo of the torsion pendulum and the mounted source mass.}
\label{fig:schematic}
\end{figure*}


%\begin{figure}[htb]
%\centering
%\includegraphics[width=0.9\linewidth]{images/spectrum.png}
%\caption[spectrum]{The rotation of the torsional oscillator is calibrated as test mass displacement (blue) and respective exerted force (light red). 
%%The spectrum shows gravitational coupling at $f_0=12.7\,$mHz modulation frequency plus the nonlinearity of the gravitational potential at $2f_0$ well above the oscillator's resonance frequency of 2.5\,mHz. Both signals are in agreement with the expected gravitational signal (dark red). 
%The measurement is limited by diurnally varying white force noise below 100\,mHz while white displacement readout noise dominates above. The torsional motion is decoupled well from other oscillator modes, starting at 500\,mHz.}
%\label{fig:spectrum}
%\end{figure}

\begin{figure*}[htb]
\centering
\includegraphics[width=0.9\linewidth]{images/spectrum_no_inset.png}
\caption[spectrum]{The rotation of the torsional oscillator measured over a period of 13.5 hours is calibrated as test mass displacement (blue) and respective exerted force (light red). 
%The spectrum shows gravitational coupling at $f_0=12.7\,$mHz modulation frequency plus the nonlinearity of the gravitational potential at $2f_0$ well above the oscillator's resonance frequency of 2.5\,mHz. Both signals are in agreement with the expected gravitational signal (dark red). 
The measurement is limited by diurnally varying white force noise below $100\,\mathrm{mHz}$ while white displacement readout noise dominates above. The torsional motion is decoupled well from other oscillator modes, starting at 0.5\,Hz.}
\label{fig:spectrum}
\end{figure*}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{images/bonfire_hot.png}
    \caption{The probability density distribution of exerted force versus source- test mass separation (a) shows the spatial non-linearity of the source-mass potential. Note that this method makes full use of our measurement data by taking into account weighting with the current noise conditions. The apparent width of the distribution is mainly given by noise at frequencies other than the modulation. (b) The actual measurement precision becomes apparent by extracting the mean of the force measured at given distances (red points) along with their standard deviation obtained by bootstrapping (red band) . A full weighted fit of the 13.5\,h long data segment with Newtonian gravity (black line) yields $G_{fit}=(5.89\pm0.20)\times10^{-11}\,\mathrm{N}\,\mathrm{m}^2/\mathrm{kg}^2$ which is in agreement with our long-term combined value (see \figref {G}). Comparison with the literature value $G_{lit}=6.67\times10^{-11}\,\mathrm{N}\,\mathrm{m}^2/\mathrm{kg}^2$ (dashed line) and our known systematic errors shows that influences other than gravity are below $10\,\%$.}
    \label{fig:bonfire}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=0.9\linewidth]{images/gravity.png}
\caption[G]{Over a stretch of three weeks during the seismically quiet Christmas season several measurement runs were conducted, with electrostatic coupling being excluded during gray periods. The dataset presented in \figref{spectrum} and \ref{fig:bonfire} is highlighted in black (run 1). The statistical error ($1\sigma$ error bar) of the best fitting Newton-like coupling of each data segment (dark lines) varies due to highly non-stationary noise in the measurement band. Combining individual measurements weighted by their respective data quality yields $G_{comb} = (6.04\pm0.06)\times10^{-11}\,\mathrm{N}\,\mathrm{m}^2/\mathrm{kg}^2$. We explicitly do not claim a significant systematic deviation from the literature value (see \cite{SI}) as the experiment and its data evaluation was mainly designed with the reduction of statistical errors in mind.}
\label{fig:G}
\end{figure*}
